Analytic results for heavy-quark contributions to charged-current DIS at NNLO

We present analytic results for the next-to-next-to-leading-order QCD corrections to heavy-quark production in charged-current deep-inelastic scattering, retaining the exact dependence on the charm quark mass. We compute the complete partonic coefficient functions for the structure functions $F_2$, $F_L$, and $F_3$ in the quark and gluon channels, including contributions with up to three heavy quarks in the final state. Working within the reverse-unitarity framework, we use integration-by-parts and canonical differential-equations techniques to express all contributions with at most two final-state heavy quarks in terms of manifestly real Goncharov polylogarithms which allow for a robust and efficient numerical evaluation. The three-heavy-quark contribution involves elliptic structures for which we give a general representation in terms of Chen iterated integrals, as well as expressions in terms of rapidly convergent expansions that are valid in the perturbative $Q\gtrsim 5~{\rm GeV}$ region and also allow for a flexible and fast numerical evaluation. We validate our results against known exact results at lower orders, massless NNLO coefficient functions, and existing leading-power expansions in the asymptotic limit where the virtuality $Q$ is much larger than the charm mass.

==> tikz/R/TBoxm2c13_111.tex <==
\begin{tikzpicture}[ >=stealth,
  inner sep=0pt, outer sep=0pt,
  shorten <=-0.55pt, shorten >=-0.55pt,
  baseline=(current bounding box.center)]
  \node[inner sep=0pt] (2) at (1.66,1.71) {};
  \node[inner sep=0pt] (e1) at (1.9,2) {};
  \node[inner sep=0pt] (5) at (0.78,1.26) {};
  \node[inner sep=0pt] (e2) at (0.3,1.26) {};
  \node[inner sep=0pt] (6) at (1.65,0.80) {};
  \node[inner sep=0pt] (7) at (1.65,1.25) {};
  \node[inner sep=0pt] (e4) at (1.9,.5) {};
  \node[inner sep=0pt] (e4u) at (2.0,.6) {};
  \node[inner sep=0pt] (e4d) at (1.8,.4) {};
  \node[inner sep=0pt] (c1) at (1.0,0.685) {};
  \node[inner sep=0pt] (c2) at (2.00,1.275) {};
  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (2) -- (e1);
  \node[font=\scriptsize] at ($ (2)!0.5!(e1) $) {};

  \draw[-, thick] (5) -- (e2);
  \node[font=\scriptsize] at ($ (5)!0.5!(e2) $) {};


  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (6) -- (e4u);
  \draw[-, thick] (6) -- (e4d);


  \node[font=\scriptsize] at ($ (6)!0.5!(e4) $) {};

  \draw[-, thick, double] (2) to (5);
  \node[font=\scriptsize] at ($ (2)!0.5!(5) $) {};

  \draw[-, thick, double] (5) -- (6);
  \node[font=\scriptsize] at ($ (5)!0.5!(6) $) {};

  \draw[-, thick] (6) -- (2);
  \node[font=\scriptsize] at ($ (6)!0.5!(2) $) {};

%  \draw[-, thick] (5) to (7);
%  \node[font=\scriptsize] at ($ (5)!0.5!(7) $) {};

  % red dashed line SSE → NNW
  \draw[-,red, thick, dashed, dash pattern=on 2pt off 1pt] (c1) to (c2);
  \node[font=\scriptsize] at ($ (c1)!0.5!(c2) $) {};

  \end{tikzpicture}

==> tikz/R/TBoxmc13_101.tex <==
\begin{tikzpicture}[
    >=stealth,
  inner sep=0pt, outer sep=0pt,
  shorten <=-0.55pt, shorten >=-0.55pt,
  baseline=(current bounding box.center)]
  \node[inner sep=0pt] (2) at (0.44,0.1) {};
  \node[inner sep=0pt] (5) at (1.44,0.1) {};
  \node[inner sep=0pt] (e2) at (1.84,0.1) {};
  \node[inner sep=0pt] (e4) at (0.00,0.1) {};
  \node[inner sep=0pt] (e2u) at (1.84,0.2) {};
  \node[inner sep=0pt] (e4u) at (0.00,0.2) {};
  \node[inner sep=0pt] (e2d) at (1.84,0.0) {};
  \node[inner sep=0pt] (e4d) at (0.00,0.0) {};

  \draw[-, thick] (e2u) to (5);
  \draw[-, thick] (e4u) to (2);
  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (e2d) to (5);
  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (e4d) to (2);
%  \draw[-, thick] (2) to (5);
  \draw[-, thick, bend left=90] (5) to (2);
  \draw[-, thick, bend left=90, double] (2) to (5);
  \draw[red, thick, dashed, dash pattern=on 2pt off 1pt]
    let \p1 = (current bounding box.north), \p2 = (current bounding box.south)
    in (0.94,\y2) -- (0.94,\y1);
\end{tikzpicture}

==> tikz/V/TBoxcvm_001.tex <==
\begin{tikzpicture}[
    >=stealth,
  inner sep=0pt, outer sep=0pt,
  shorten <=-0.55pt, shorten >=-0.55pt,
  baseline=(current bounding box.center)]
  \node[inner sep=0pt] (2) at (0.44,0.1) {};
  \node[inner sep=0pt] (5) at (1.44,0.1) {};
  \node[inner sep=0pt] (e2) at (1.84,0.1) {};
  \node[inner sep=0pt] (e4) at (0.00,0.1) {};
  \node[inner sep=0pt] (e2u) at (1.84,0.2) {};
  \node[inner sep=0pt] (e4u) at (0.00,0.2) {};
  \node[inner sep=0pt] (e2d) at (1.84,0.1) {};
  \node[inner sep=0pt] (e4d) at (0.00,0.1) {};

%  \draw[-, thick] (e2u) to (5);
%  \draw[-, thick] (e4u) to (2);
%  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (e2d) to (5);
%  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (e4d) to (2);
%  \draw[-, thick] (2) to (5);
  \draw[-, thick, bend left=90, double] (5) to (2);
  \draw[-, thick, bend left=90, double] (2) to (5);
%  \draw[red, thick, dashed, dash pattern=on 2pt off 1pt]
%    let \p1 = (current bounding box.north), \p2 = (current bounding box.south)
%    in (0.94,\y2) -- (0.94,\y1);
\end{tikzpicture}

==> tikz/V/TBoxcvm_011.tex <==
\begin{tikzpicture}[
    >=stealth,
  inner sep=0pt, outer sep=0pt,
  shorten <=-0.55pt, shorten >=-0.55pt,
  baseline=(current bounding box.center)]
  \node[inner sep=0pt] (2) at (0.44,0.1) {};
  \node[inner sep=0pt] (5) at (1.44,0.1) {};
  \node[inner sep=0pt] (e2) at (1.84,0.1) {};
  \node[inner sep=0pt] (e4) at (0.00,0.1) {};
  \node[inner sep=0pt] (e2u) at (1.84,0.2) {};
  \node[inner sep=0pt] (e4u) at (0.00,0.2) {};
  \node[inner sep=0pt] (e2d) at (1.84,0.1) {};
  \node[inner sep=0pt] (e4d) at (0.00,0.1) {};

%  \draw[-, thick] (e2u) to (5);
%  \draw[-, thick] (e4u) to (2);
  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (e2d) to (5);
  \draw[-, thick,decorate, decoration={snake, amplitude=.5pt, segment length=3pt}] (e4d) to (2);
%  \draw[-, thick] (2) to (5);
  \draw[-, thick, bend left=90, double] (5) to (2);
  \draw[-, thick, bend left=90] (2) to (5);
%  \draw[red, thick, dashed, dash pattern=on 2pt off 1pt]
%    let \p1 = (current bounding box.north), \p2 = (current bounding box.south)
%    in (0.94,\y2) -- (0.94,\y1);
\end{tikzpicture}
